Learning Intrinsic Images for Clothing

Reconstruction of human clothing is an important task and often relies on intrinsic image decomposition. With a lack of domain-specific data and coarse evaluation metrics, existing models failed to produce satisfying results for graphics applications. In this paper, we focus on intrinsic image decomposition for clothing images and have comprehensive improvements. We collected CloIntrinsics, a clothing intrinsic image dataset, including a synthetic training set and a real-world testing set. A more interpretable edge-aware metric and an annotation scheme is designed for the testing set, which allows diagnostic evaluation for intrinsic models. Finally, we propose ClothInNet model with carefully designed loss terms and an adversarial module. It utilizes easy-to-acquire labels to learn from real-world shading, significantly improves performance with only minor additional annotation effort. We show that our proposed model significantly reduce texture-copying artifacts while retaining surprisingly tiny details, outperforming existing state-of-the-art methods.

==> dataset.tex <==
%!TEX root=main.tex

\begin{figure}
\centering
% \vspace{-2mm}
\includegraphics[width=\textwidth]{src/CloIntrinsics.pdf} 
\vspace{-6mm}
\caption{\footnotesize\textbf{Visualization of CloIntrinsics Training Set. } 
We collect 3D clothing models designed by artists and put them on avatars. 
The pose of avatars is changed to simulate various wrinkle patterns in real world, and the texture patterns are changed to generate diverse reflectance. 
These models are rendered with different viewpoints and lighting and form the synthetic training set. 
}
\label{fig:CloIntrinsics}
\vspace{-3mm}
\end{figure}

\vspace{-3mm}
\section{CloIntrinsics Dataset} 
\label{sec:dataset}
\vspace{-1mm}
% \INFO{
% Sketch: Introduce the datasets. 

% Intuition as intro: why datasets? 

% subsec1: synthetic training set

% subsec2: testing set and metric definition 
% }

% Since data is the bottleneck for intrinsic models, 
% As far as we know, there's no intrinsic image dataset in clothing domain. 
To relieve the data-hungry situation and improve the relatively rough evaluation metrics for intrinsic models, we propose Clothing Intrinsic Images (CloIntrinsics) Dataset, including a synthetic training set and a real-world testing set. 
% We carefully design the annotation scheme and propose a diagnostic metric for intrinsic models. 
\vspace{-3mm}
\subsection{Synthetic Training Set}
\vspace{-1mm}
Although largescale synthetic datasets for animated film \cite{butler2012naturalistic} and indoor scenes \cite{li2018cgintrinsics} exist, we believe clothes generally have different priors in the shape deformation and texture patterns, and the in-domain data will surely improve the performance of intrinsic image decomposition models. 
The key is to render as realistic as possible clothing data. 
We choose to use fashion design software CLO3d \cite{Cloth3D}, which produce realistic 3D clothing models with garment flats, and render the 3D models with Blender \cite{Blender}. 
To simulate real world conditions better, as shown in Fig.~\ref{fig:CloIntrinsics}, the training set contains diversity in the following aspects. 

\vspace{1mm}
\noindent\textbf{Shape.} 
% Real-world clothing images can have complex and detailed shapes, and recovering the correct shading effect is crucial in many applications. 
The variety of clothing shapes generally comes from different clothing types, and the shape deformation causes by the wearer's poses. 
To cover common clothing types like T-shirt, jacket, dress, suit, etc., CloIntrinsics collects 80 3D clothing models designed by artists. 
To include diverse wrinkle patterns, we change the poses of avatars and simulate the deformation of clothing. 
In this way, it collects diverse shape patterns for clothing. 
As a further augmentation, we render these models in different viewpoints to get more diverse images. 

\vspace{1mm}
\noindent\textbf{Reflectance.} 
The complex texture is among the challenges for clothing intrinsic image decomposition and it's vital to render a dataset with diverse texture. 
To address this, we build a database with around 200 texture patterns. 
As fashion design software like CLO3d designs clothing with garment flats, we change the texture pattern of garment flats for each 3d clothing models, and thus increase diversity in reflectance. 

\vspace{1mm}
\noindent\textbf{Lighting.}
Real world images generally contain complex lighting conditions. 
In addition to global ambient lights, we generate random light sources during rendering to improve the complexity of lighting conditions. 
The light sources consist of one hemisphere lighting and 10 to 20 point lights randomly sampled on the upper hemisphere, with random intensity. 

% \vspace{1mm}
The data generation pipeline is shown in Fig.\ref{fig:CloIntrinsics}. We first collect 3D clothing models designed by artists. We then put them on avatars and simulate the shape deformation caused by pose changes. Different texture patterns are used to include diverse reflectance map. We finally render the models with different viewpoints and lighting conditions. 
With the settings above, we finally raytraced 5K clothing images with paired intrinsic components at the resolution of 1024x1024. 
% These data contain prior knowledge in clothing domain and improve the performance of intrinsic image decomposition models. 

\vspace{-3mm}
\subsection{Real World Testing Set} 
\vspace{-1mm}
To convincingly reflect the real-world performance, we choose to evaluate our model on real world clothing images instead of synthetic data. 
We randomly select 500 clothing images from Paper Doll Dataset \cite{yamaguchi2013paper}, and ask human experts with knowledge background in intrinsic images to annotate \emph{regions} and \emph{edges} of interest. 
The proposed edge-aware metric significantly improves the interpretability and expressiveness of existing metrics. 
% To improve the interpretability and expressive of existing metrics, we propose a novel edge-aware metric and design an corresponding annotation scheme. 
The details are included in Sec.~\ref{sec:metric} below. 



\vspace{-3mm}
\section{Edge-Aware Metric}
\label{sec:metric}
\vspace{-1mm}

% Generally speaking, a good evaluation metric should reflect how models perform against common artifacts. 
The task of intrinsic image decomposition requires to distinguish whether the local pixel value changes, i.e. edges, are caused by the change of reflectance or shading. 
Also, the edge performance of intrinsic image decomposition models is crucial in many graphics applications, and deserves special attention. 
However, current popular evaluation metrics are not able to evaluate edge performance in an interpretable way, and thus not expressive to show how models perform against artifacts. 
For instance, the major challenge for intrinsic models is the texture-copying artifact, which often happens on edges due to the entanglement of intrinsic components. The sparse WHDR metric in IIW dataset \cite{bell2014intrinsic} and AP used in SAW dataset \cite{kovacs2017shading} are not able to reflect this artifact. 

% \TODO{[explain more in supp? ]} 
For edges, component entanglement often happens, when the model fails to determine whether the change is caused by reflectance or shading. Edges can result from the change of reflectance only, shading only or both. To evaluate the predictions, we need to have better understanding on what happens around these edges. 
In addition to edges with abrupt local changes, we're also interested in how well the prediction fits the groundtruth around the relatively flat \emph{regions}, e.g. in a constant-reflectance region, reflectance value shouldn't change while shading values should fit tightly to the changes. 

With the analysis above, we need to first design a data annotation scheme to annotate edges and regions of interest (Sec.~\ref{sec:annotation}). 
On top of the annotation, we design an diagnostic edge-aware metric to maximally reflect how model behaves (Sec.~\ref{sec:metric_design}). 
% both edge-based metrics and region-based metrics. 
% To improve the interpretability of evaluation metrics, we design a data annotation scheme and an edge-aware metric. 
% The common artifacts mainly lie in two categories: component entanglement and global inconsistency. 
% Component entanglement often happens on edges, when the decomposition fails to determine whether the change is caused by reflectance or shading. 
% For distant pixels that should have similar reflectance or shading, global inconsistency often happens due to the scale ambiguity of intrinsic images. 


\begin{figure}[t]
\centering
\vspace{-4mm}
\includegraphics[width=\linewidth]{src/annotation.pdf} 
\vspace{-8mm}
\caption{\footnotesize\textbf{Visualization of Annotation Result. } 
The left is RGB image and the right is the annotation results visualized on grayscale image. 
Red indicates edges caused only by shading ($\mathcal{E}_\text{S}$) and dark green shows edges caused only by reflectance ($\mathcal{E}_\text{R}$). Other colors indicate constant-reflectance regions $\{\mathcal{R}_c\}$. 
Best viewed zooming in. 
}
\label{fig:annotation}
\vspace{-4mm}
\end{figure}

\vspace{-3mm}
\subsection{Data Annotation Scheme}
\label{sec:annotation}
\vspace{-1mm}
% As discussed above, to better evaluate the common artifacts of intrinsic models,
For CloIntrinsics testing set, we need data annotation on both edges $\mathcal{E}$ and regions $\mathcal{R}$ of interest. % $\{\mathcal{E}, \mathcal{R}\}$. 
Considering the difficulty and accuracy during annotation, we propose to focus on annotating constant-reflectance regions and edges caused by reflectance only or shading only. 

Specifically, region annotation $\mathcal{R} = \{\mathcal{R}_c | c=1,2,\cdots, C\}$ contains several regions $\mathcal{R}_c$ and elements in $\mathcal{R}_c$ have the same reflectance $c$. The annotators are asked to find pixels with intrinsically the same ``color'', i.e. the same reflectance, and annotate them with points or polygons. Instead of including comparison with inequal reflectance values, annotators can easily annotate more precise results. 

Edge annotation $\mathcal{E} = \{\mathcal{E}_\text{R}, \mathcal{E}_\text{S} \}$ is a subset of $\mathcal{E}_\text{Canny}$, which is edges detected by Canny algorithm \cite{canny1986computational}. 
$\mathcal{E}_\text{R}, \mathcal{E}_\text{S}$ denotes the edges caused by reflectance only and shading only, respectively. 
As we can use $\mathcal{E}_\text{S} = \mathcal{E}_\text{Canny} \cap \mathcal{R}$ to get the edges caused by shading, where $\mathcal{R}$ is the constant-reflectance regions we already annotated, 
we can simplify the annotation process and only need to annotate the edges caused by reflectance $\mathcal{E}_\text{R}$. 
To annotate $\mathcal{E}_\text{R}$, we design a user interface which shows Canny edges, and ask the annotators to add scribbles to the edges caused only by reflectance. 

% To make the edge annotation more precise, we implement a optimization-based algorithm based on the framework of \cite{zhao2012closed}. It uses Retinex constraint \cite{land1971lightness1} and enforce shading image to be smooth around annotated $\mathcal{E}_\text{R}$. 
% The decomposition results are displayed to the annotators, giving them a chance to make sure the annotation can lead to locally satisfying results. 
% Some annotation examples are shown in Fig.~\ref{fig:annotation}. 
The annotation collection pipeline includes data annotation and data verification, conducted by three annotators with background in intrinsic images. 
For data annotation, we ask two of the annotators to annotate the images twice. They are asked to only annotate the confident parts. 
The annotation will then be combined, and another inspector will verify the annotation. 
We noticed that it's hard for the inspector to find mistakes directly by watching the edge annotation, but it's easier for the inspector to judge whether reflectance and shading are well behaved. 
Based on this observation, we incorporate an interactive method \cite{bousseau2009user} for annotation inspection. 
Specifically, We use our edge annotation as the prior to solve for intrinsic images, and the results will be displayed to the annotator. 
Only when our annotation leads to plausible decomposition results can we assume the annotation is reliable. 
With the above professional annotation procedure, we obtained high quality annotation on real-world images. 


\vspace{-3mm}
\subsection{Metric Design}
\label{sec:metric_design}
\vspace{-1mm}
With region annotation $\{\mathcal{R}_c | c=1,2,\cdots, C\}$ and edge annotation $\{\mathcal{E}_\text{R}, \mathcal{E}_\text{S} \}$, we define metric for region performance and edge performance separately. 

\vspace{1mm}
\noindent\textbf{Region reflectance metric. }
Pixels with the same reflectance should have similar values in the decomposition results. 
Given the predicted reflectance $\hat{R}$, we calculate the variance within each annotated region as a metric to evaluate the performance of predicted reflectance. 
Specifically, for each region $\mathcal{R}_c$, we first normalize the mean to $1$ considering the ambiguity in scale, 
\begin{equation}
	\tilde{R}_{i, j} = \frac{|\mathcal{R}_c|}{\sum_{(m, n) \in \mathcal{R}_c} \hat{R}_{m, n}} \ \hat{R}_{i, j}. 
	\label{eq:norm}
\end{equation}
Then we compute the variance as the error measure of reflectance
% \begin{equation}
% 	Var(\mathcal{R}_c) = \frac{1}{|\mathcal{R}_c|} \sum_{(i, j) \in \mathcal{R}_c} (\tilde{R}_{i, j} - 1)^2,
% \end{equation}
\begin{equation}
	\text{RegionError}_\text{R} = \frac 1C \sum_{c=1}^{C} \frac{1}{|\mathcal{R}_c|} \sum_{(i, j) \in \mathcal{R}_c} (\tilde{R}_{i, j} - 1)^2. 
\end{equation}

\vspace{1mm}
\noindent\textbf{Region shading metric. }
Within each constant reflectance region $\mathcal{R}_c$, we can assume the reflectance is constant and compute the estimated groundtruth shading $S_c$, which is RGB image divided by reflectance. 
% $\hat{S}_{i, j}\frac{I_{i, j}}{\hat{R}_{i, j}}, (i, j) \in \mathcal{R}_c$
Given the predicted shading $\hat{S}$, we compute scale-invariant mean square error (si-MSE) as a metric to evaluate global shading performance, 
\begin{equation}
	\text{si-MSE}_{\mathcal{R}}(\hat{X}, X) = \frac{1}{|\mathcal{R}|} \sum_{(i, j) \in \mathcal{R}} ||\alpha\hat{X}_{i,j} - X_{i,j}||^2,
\end{equation}
where $\alpha = \arg\min \sum_{(i, j) \in \mathcal{R}} ||\alpha\hat{X}_{i,j} - X_{i,j}||^2$, and
\begin{equation}
	\text{RegionError}_\text{S} = \frac{\sum_{c=1}^{C} \text{si-MSE}_{\mathcal{R}_c}(\hat{S}, S_c)}{\sum_{c=1}^{C} \text{si-MSE}_{\mathcal{R}_c}(\mathbf{0}, S_c) }
\end{equation}
where we use a relative error similar to \cite{grosse2009ground}. 
Considering that the estimated shading $S_c$ is not exactly the ground truth, we don't accumulate the part of error when the prediction error is within the range of $\pm 5\%$. 

\vspace{1mm}
\noindent\textbf{Edge metric. }
The most common artifact for edges is component entanglement. 
With edge annotation $\{\mathcal{E}_\text{R}, \mathcal{E}_\text{S} \}$, we're able to evaluate model performance in an more interpretable way. 
Ideally, the predicted reflectance $\hat{R}$ should change around $\mathcal{E}_\text{R}$ but not $\mathcal{E}_\text{S}$. 
Similarly, the predicted shading $\hat{S}$ should change around $\mathcal{E}_\text{S}$ but not $\mathcal{E}_\text{R}$. 
We use local gradient magnitude to indicate the local changes, and assume it changes when local gradient magnitude is larger than a threshold $\tau$. 
We first normalize in the same way as in Eq.~\ref{eq:norm} and get $\tilde{R}$ and $\tilde{S}$. 
Then, to indicate how well the predicted results agrees with the annotation, we define the accuracy of reflectance at $\mathcal{E}_\text{S}$ and the accuracy of shading at $\mathcal{E}_\text{R}$ as follows
\begin{equation}
	\text{Acc}_\text{R}^{(\mathcal{E}_\text{S})} = 
	\frac{\sum_{(i, j) \in \mathcal{E}_\text{S}} \mathbbm{1}\big( ||\nabla \tilde{R}_{i, j}|| < \tau \big) }{|\mathcal{E}_\text{S}|}, \ 
	\text{Acc}_\text{S}^{(\mathcal{E}_\text{R})} = 
	\frac{\sum_{(i, j) \in \mathcal{E}_\text{R}} \mathbbm{1}\big( ||\nabla \tilde{S}_{i, j}|| < \tau \big) }{|\mathcal{E}_\text{R}|},
\end{equation}
where $\mathbbm{1}(\cdot)$ is the indicator function. 
The accuracies defined above directly indicate how reflectance and shading entangle with each other, making it interpretable and diagnostic. 
Similarly, we can also define the accuracy of reflectance at $\mathcal{E}_\text{R}$ as $\text{Acc}_\text{R}^{(\mathcal{E}_\text{R})}$, and the accuracy of shading at $\mathcal{E}_\text{S}$ as $\text{Acc}_\text{S}^{(\mathcal{E}_\text{S})}$, 
\begin{equation}
	\text{Acc}_\text{R}^{(\mathcal{E}_\text{R})} = 
	\frac{\sum_{(i, j) \in \mathcal{E}_\text{R}} \mathbbm{1}\big( ||\nabla \tilde{R}_{i, j}|| > \tau \big) }{|\mathcal{E}_\text{R}|}, \ 
	\text{Acc}_\text{S}^{(\mathcal{E}_\text{S})} = 
	\frac{\sum_{(i, j) \in \mathcal{E}_\text{S}} \mathbbm{1}\big( ||\nabla \tilde{S}_{i, j}|| > \tau \big) }{|\mathcal{E}_\text{S}|}.
\end{equation}
We finally use weighted harmonic mean as the metric for edge performance, 
\begin{equation}
	F_\text{R} = \frac{w_1 + w_2}{ \frac{w_1}{\text{Acc}_\text{R}^{(\mathcal{E}_\text{S})}} + \frac{w_2}{\text{Acc}_\text{R}^{(\mathcal{E}_\text{R})}}}, \ 
	F_\text{S} = \frac{w_1 + w_2}{ \frac{w_1}{\text{Acc}_\text{S}^{(\mathcal{E}_\text{R})}} + \frac{w_2}{\text{Acc}_\text{S}^{(\mathcal{E}_\text{S})}}}, 
	\label{eq:edge_metric}
\end{equation}
% where $F_\text{R}$ and $F_\text{S}$ 
indicating edge performance of reflectance and shading respectively. 



In summary, for the real-world testing set, we use $\text{RegionError}_\text{R}$, $\text{RegionError}_\text{S}$ to evaluate generally how well the predicted intrinsic images fit to the groundtruth. 
For common component entanglement artifacts, we use $\text{F}_\text{R}$ and $\text{F}_\text{S}$ to evaluate the edge performance of intrinsic models. By looking at $\text{Acc}_\text{R}^{(\mathcal{E}_\text{R})}, \text{Acc}_\text{R}^{(\mathcal{E}_\text{S})}, \text{Acc}_\text{S}^{(\mathcal{E}_\text{R})}, \text{Acc}_\text{S}^{(\mathcal{E}_\text{S})}$, we can learn diagnostic information on how model behaves around edges. 
% \TODO{more intuition here!!}




==> intro.tex <==
%!TEX root=main.tex
\vspace{-4mm}
\section{Introduction}
\label{sec:intro}
\vspace{-1mm}

% % TODO!!!
% \begin{figure}[t!]
% \centering
% \vspace{-1mm}
% \includegraphics[width=0.9\linewidth]{src/teaser.pdf} 
% \vspace{-3mm}
% \caption{\footnotesize\textbf{Clothing intrinsic image decomposition and image editing.} 
% On these challenging cases, we perform color style editing and colorize the clothing with a single color. Our ClothInNet model significantly reduces texture-copying artifacts and thus allows realisitic editing. 
% }
% \label{fig:teaser}
% \vspace{-6mm}
% \end{figure}

Analysis and reconstruction of human clothing texture is an important task for computer vision and computer graphics, yet still receiving little specialized attention. 
In recent works, intensive research efforts have been focus on analysis of human appearance, e.g., reconstruction of 3D human~\cite{imber2014intrinsic,wu2011shading,guo2017real} and editing or synthesis of human characters \cite{meka2016live,li2013capturing}. Many of these methods leverage intrinsic image decomposition \cite{imber2014intrinsic} and related techniques like shape from shading \cite{wu2011high} to decompose texture information into reflectance, geometry and lighting information. 
As a fact that clothing covers most of the surface area of people in daily life, it is vital to focus on clothing texture.
% However, all these methods regard the human texture as a whole, and do not exclusively focus on analysis of human clothing appearance. 

In this paper, we consider the problem of intrinsic image decomposition for human clothing. 
% Intrinsic image decomposition was extensively studied in the past 40 years, 
Driven by the real-world applications like image editing and benefits for other vision tasks such as 3D reconstruction and image segmentation, intrinsic image decomposition was extensively studied but remains a challenging task due to its ill-posed nature. 
It aims to decompose a given image $I$ into corresponding intrinsic images, usually the reflectance image $R$ encoding the surface albedo and the shading image $S$ encoding illumination conditions, satisfying Hadamard product $I = R \odot S$. 

Early work designed energy terms based on priors and formulated the task as an energy minimization problem \cite{land1971lightness,omer2004color,bousseau2009user,rother2011recovering,garces2012intrinsic,zhao2012closed,liao2013non}. 
However, they usually suffer from large computational cost, and the proposed priors are not always true due to the complex conditions of wild images. 
An attractive alternative is to exploit the powerful CNNs and learn the decomposition in a data-driven manner \cite{narihira2015direct,shi2017learning,nestmeyer2017reflectance,baslamisli2018cnn,fan2018revisiting,cheng2018intrinsic,li2018cgintrinsics}. 
However, different from other vision tasks, intrinsic images are extremely hard to annotate. 
% This is because human can only provide relative comparison instead of dense annotation. 
Existing largescale datasets are either synthetic data with dense groundtruth \cite{butler2012naturalistic,li2018cgintrinsics,baslamisli2018joint,baslamisli2018cnn} or real world images with sparse annotation \cite{bell2014intrinsic,kovacs2017shading}. 
With the data-hungry bottleneck, efficient usage of diverse data sources \cite{janner2017self,li2018learning,ma2018single} for indirect supervision becomes more important. 

Recent state-of-the-art methods with higher benchmark scores still suffer from severe texture-copying artifacts, stopping them from real world applications. 
The bottleneck mainly lies in \emph{metric} and \emph{data}. 
With research progress in this field, existing popular evaluation metrics \cite{bell2014intrinsic,kovacs2017shading,grosse2009ground} can easily get cheated and no longer truly reflect real performance \cite{nestmeyer2017reflectance}. Models with better quantitative scores may perform qualitatively worse, making it urgent to have a more expressive metric. 
For the data-hungry bottleneck, to gain enough supervision for this ill-posed task, it's essential to intelligently utilize diverse data sources.% to further improve current models' performance. 
% Also, the evaluation metrics for intrinsic images seldom include edge performance and are not interpretable. 
% With the coarse evaluation, a model with high scores can still produce fairly noisy results. 
% fail on challenging cases like clothing images, which usually contain rather detailed shape and complex texture. The predicted intrinsic images suffers from severe texture-copying artifacts, stopping them from real world applications. 


In this paper, we address the weaknesses mentioned above and aim to improve the performance on the challenging clothing images. 
% of intrinsic image decomposition and have comprehensive 
% in \emph{data}, \emph{metric} and \emph{model}. 
First, to relieve the data-hungry situation of clothing intrinsic images, we collected CloIntrinsics dataset, with a rendered synthetic clothing image training set and a testing set with real world clothing images. Professional software for clothing design \cite{Cloth3D} is used to simulate as realistic as possible clothing models. 
% which are then rendered with diverse texture, different viewpoints and random illumination conditions. 
Second, we carefully designed an annotation scheme and propose a new edge-aware metric to evaluate intrinsic image decomposition models. It targets at common artifacts on real world images and provide interpretable and diagnostic feedback. 
% An annotation scheme is carefully designed to give much clearer indications on common artifacts. 
% The testing set, with a carefully designed annotation scheme, allows to evaluate model performance on both regions and edges. The diagnostic metrics are able 
Third, we propose ClothInNet, a simple but effective model for clothing intrinsic image decomposition. 
In this model, we incorporate the large number of easy-to-acquire \emph{single-color clothing} images as additional supervision sources. 
These images reflect the probability distrubution of real-world shading data, which is learned by the network in an adversarial manner. 
% and utilize an adversarial learning module to enforce the output shading to follow the distribution of real-world shading. 
Additionally, a novel loss term is proposed to apply local gradient constraint on reflectance images and significantly improves performance. 
% It carefully utilized the priors of clothes, and significantly improves the performance with only minor additional annotation. 

The contribution of this paper can be summarized as: 
\vspace{-2mm}
\begin{packed_item}
	\item a clothing intrinsic image dataset, including a synthetic training set and a real world testing set (Sec.~\ref{sec:dataset}),
	\item a diagnostic metric to evaluate intrinsic image decomposition models (Sec.~\ref{sec:metric}), 
	\item a model to distil real-world shading distribution and carefully designed loss terms to apply exclusive gradient constraints on albedo (Sec.~\ref{sec:method}).
	 % from easy-to-acquire labels and a simple but effective CNN model utilizing these data  
	% proposed a weakly supervised model based on adversarial learning, which achieves better shading performance on clothing images. 
\end{packed_item}

% For single-image IID, this paper proposed a weakly supervised model based on adversarial learning, which achieves better performance on clothing images.
% This method carefully utilized the priors of clothes, and significantly improves the performance without the need for complex data annotation. 
% The weakly supervised adversarial learning approach may also inspire tasks in other fields.

% Additionally, this paper also rendered a large-scale clothing image dataset for supervised model. 
% Professional software for clothing design is used to simulate the shape deformation of clothing with different poses. 
% The generated 3D clothing models are then rendered with diverse texture, different viwepoints and random illumination conditions. 
% The dataset could introduce strong supervision to deep learning models, and significantly improved the quality of the decomposition results. 





==> related.tex <==
%!TEX root=main.tex

\section{Related Work}

% The research on intrinsic image originates from the study of human vision in the 1970s. Visual system is a crucial part of human perception of the external environment. The visual effects of objects observed by human beings are affected by many factors, such as material, texture, shape, position and color of light source, and position of the observer. 
% From experimental results, scientists observed that the human visual system has the ability to separate light and color. 
% To explain this phenomenon, Land \etal \cite{land1971lightness} proposed Retinex theory on human color perception. 
% Barrow \etal \cite{barrow1978recovering} then formally proposed the task of intrinsic image decomposition.
 % which decomposes a color image into different attributes and represents it as a series of intrinsic images. 
\vspace*{-1mm}
\textbf{Intrinsic Image Decomposition Methods.}
Intrinsic image decomposition algorithms can be roughly divided into two categories: (1) optimization algorithms based on hand-crafted priors and (2) data-driven learning-based methods. 
Early methods usually formulate this task as an optimization problem \cite{land1971lightness,omer2004color,shen2008intrinsic,bousseau2009user,rother2011recovering,garces2012intrinsic,zhao2012closed,liao2013non,barron2014shape}. 
The main idea is to design a specific energy function with prior knowledge observed from image data, and then solve for the intrinsic images by minimizing the energy function. 
% Among these, Retinex theory \cite{land1971lightness} proposed by Land \etal is one of the most important priors, assuming large image discontinuities result from the changes of reflectance while small changes come from shading. 
% Some straight-forward priors include (1) neighbor pixels may have similar reflectance and shading values, (2) reflectance is piece-wise constant, and (3) the number of reflectance value in an image is relatively sparse. 
% Apart from these, one of the most important observation is Retinex theory \cite{land1971lightness}. 
% Retinex algorithm assumes that the larger discontinuities in the image are usually related to the change of reflectance while smaller changes are mainly caused by shading. 
% According to Grosse \etal \cite{grosse2009ground}, Retinex algorithm and its variants are still among the most successful intrinsic image decomposition algorithms. 
% Retinex theory produces priors locally, lacking the ability to deal with non-local artifacts. 
% Zhao \etal \cite{zhao2012closed} proposed non-local texture constraints assuming regions with similar texture properties should also have similar reflectance. 
% The model jointly optimizes different types of energy and can efficiently generate a closed-form solution. 
% Researchers also studied incorporating additional inputs to increase the quality of intrinsic decomposition models. 
% Bousseau \etal \cite{bousseau2009user} proposed an interactive intrinsic deomposition method, which utilizes human clicks to refine the quality of decomposition results. 
% The above-mentioned optimization algorithms can already generate reasonable results with simple object images or scenes. 
But real-world images can not fully meet these hand-crafted priors, and thus severe artifacts would occur. 
% Also, optimization-based methods generally suffer from high computational cost, making them less appealing for applications in real-time. 
% In recent years, a large number of data-driven learning-based methods, especially deep learning methods, have emerged in the field of computer vision and computer graphics. 
% Researchers also proposed learning-based methods for intrinsic image decomposition. 
With fruitful achievements in other vision tasks, a promising alternative is to learn data-driven features, leveraging the powerful CNNs for feature extraction \cite{narihira2015direct,shi2017learning,nestmeyer2017reflectance,janner2017self,li2018learning,ma2018single,fan2018revisiting,cheng2018intrinsic,lettry2018darn,sengupta2019neural,yu2019inverserendernet}. 
These works generally consumes RGB images as input and uses a CNN to predict one or both intrinsic images. 
Proposed methods like mirror-link architecture \cite{shi2017learning}, post-processing \cite{nestmeyer2017reflectance}, intermediate representations \cite{janner2017self} and adversarial module \cite{lettry2018darn} are shown to improve the results. 
% DirectIntrinsics\cite{narihira2015direct} proposed the Multiscale CNN Regression method and directly predict reflectance and shading from RGB. 
% Shi \etal\cite{shi2017learning} employed a mirror-link CNN architecture to predict intrinsic images and expanded to non-Lambertian settings. 
% Nestmeyer \etal\cite{nestmeyer2017reflectance} designed a CNN fully trained with sparse annotation, and found that traditional filtering methods with strong prior could still significantly increase the performance of CNN outputs. 
To handle the scarcity in the amount and domain of annotated data, recent research shifts the focus to 
% generalization ability and seek for 
indirect sources of supervision, including self-supervision \cite{janner2017self}, shared modules across datasets \cite{fan2018revisiting}, differentiable renderer \cite{sengupta2019neural,yu2019inverserendernet}, multiview images \cite{duchene2015multi,ma2018single} and multi-illumination sequences depicting the same scene \cite{lettry2018unsupervised,li2018learning,bi2018deep}. 
% \cite{janner2017self} explored using self-supervision for generalization and \cite{fan2018revisiting} proposed a network with modules that can largely shared across datasets. 
% \cite{lettry2018unsupervised,li2018learning,bi2018deep} employed the image sequences depicting the same scene but under different illumination as training data, and thus learn without ground truth decomposition. 
% \cite{duchene2015multi,ma2018single} leveraged multiview images of the scene for 3D geometry recovery to better understanding the intrinsic and lighting information.  
% \cite{sengupta2019neural,yu2019inverserendernet} explores differentiable renderer and use self-supervision to train intrinsic image decomposition models. 
However, current state-of-the-art models still generates severe artifacts for richly textured clothing images. 
The major problem is that we can't densely annotate real-world images, thus lacking the knowledge of real-world intrinsic images. 
Our proposed method utilizes clothing priors to learn real-world shading distribution and proposes a novel gradient constraint loss to address this. 
% Our ClothInNet model, with an adversarial module, can utilize easy-to-annotate labels to efficiently acquire real-world shading images. Different from \cite{lettry2018darn} in design, the adversarial module is employed to learn real-world shading distribution. 

\noindent\textbf{Intrinsic Images Datasets.}
Unlike other vision tasks, it's difficult to obtain largescale densely annotated intrinsic images, as people can't directly annotate the absolute value of reflectance and shading. 
% Also, many people may never ``see'' the reflection and shading images in their life, and this also bring great challenges to accurate data collection. 
Existing largescale datasets lie in two categories: (1) real-world images with sparse annotation and (2) synthetic data with dense groundtruth. 
% A more practical compromise is to annotate the relative comparision of pixel pairs. 
Intrinsic Images in the Wild (IIW) dataset \cite{bell2014intrinsic} provides sparse annotation for the pairwise comparison of reflectance on real world scene images. 
Shading Annotations in the Wild (SAW) dataset \cite{kovacs2017shading} provides additional sparse shading annotation on the same image data. 
However, due to the sparse labeling, the data itself is difficult to train a high-performance CNN model \cite{narihira2015direct,nestmeyer2017reflectance}. 
Synthetic datasets such as MPI Sintel \cite{butler2012naturalistic}, ShapeNet \cite{chang2015shapenet} and CGIntrinsics  \cite{li2018cgintrinsics} are also popular for training CNNs with dense supervision. 
% \cite{baslamisli2018joint} also proposed to jointly learn intrinsic images and semantic segmentation. 
But synthetic data essentially suffer from a domain gap and will affect the performance on real world data. 
% But people can easily tell apart real world images from CG rendered data, indicating a gap between their distribution. 
% The bottleneck for current learning based methods is the lack of data. 
As far as we know, CloIntrinsics dataset we propose in this work is the first intrinsic image dataset in clothing domain. 
With diverse shape deformation, lighting and texture, CloIntrinsics improves current models to produce tightly fitted predictions. 

\noindent\textbf{Intrinsic Image Metrics.}
In addition to qualitative comparison, quantitative metrics on real world datasets facilitate evaluation and comparison of intrinsic image decomposition algorithms. 
MIT Intrinisic Images dataset \cite{grosse2009ground} provides dense groundtruth intrinsic images for 20 objects, which enables quantitative comparison of existing algorithms. 
% Considering the scale ambiguity of intrinsic images, 
It uses scale-invariant mean square error as the quantitative metric. % for intrinsic algorithms. 
For real-world scene images, IIW dataset \cite{bell2014intrinsic} employs weighted human disagreement rate as a metric for reflectance, which tells how well the predicted results agrees with the sparse human annotation. 
SAW dataset \cite{kovacs2017shading} classifies the shading into smooth and non-smooth, and uses precision-recall curve to evaluate the results. 
These existing metrics are coarse and lack interpretable evaluation on edge performance. We contribute an annotation scheme and metric to address these problems. 












